Delay and Overhead Efficient Transmission Scheduling for Federated Learning in UAV Swarms

This paper studies the wireless scheduling design to coordinate the transmissions of (local) model parameters of federated learning (FL) for a swarm of unmanned aerial vehicles (UAVs). The overall goal of the proposed design is to realize the FL training and aggregation processes with a central aggregator exploiting the sensory data collected by the UAVs but it considers the multi-hop wireless network formed by the UAVs. Such transmissions of model parameters over the UAV-based wireless network potentially cause large transmission delays and overhead. Our proposed framework smartly aggregates local model parameters trained by the UAVs while efficiently transmitting the underlying parameters to the central aggregator in each FL global round. We theoretically show that the proposed scheme achieves minimal delay and communication overhead. Extensive numerical experiments demonstrate the superiority of the proposed scheme compared to other baselines.

==> references.tex <==
@article{qu_decentralized_2021,
    title = {Decentralized Federated Learning for {UAV} Networks: {Architecture}, Challenges, and Opportunities},
    author = {Qu, Yuben and Dai, Haipeng and Zhuang, Yan and Chen, Jiafa and Dong, Chao and Wu, Fan and Guo, Song},
    year = {2021},
    month = nov,
    journal = {IEEE Netw.},
    volume = {35},
    number = {6},
    pages = {156--162},
    doi = {10.1109/MNET.001.2100253}
}

@inproceedings{tang_communication-efficient_2020,
    title = {Communication-Efficient Decentralized Learning with Sparsification and Adaptive Peer Selection},
    booktitle = {Proc. Int. Conf. Distrib. Comput. Syst. (ICDCS)},
    author = {Tang, Zhenheng and Shi, Shaohuai and Chu, Xiaowen},
    year = {2020},
    month = nov,
    pages = {1207--1208},
    doi = {10.1109/ICDCS47774.2020.00153}
}

@article{feng_blockchain-empowered_2022,
    title = {Blockchain-Empowered Decentralized Horizontal Federated Learning for {5G}-Enabled {UAVs}},
    author = {Feng, Chaosheng and Liu, Bin and Yu, Keping and Goudos, Sotirios K. and Wan, Shaohua},
    year = {2022},
    month = may,
    journal = {IEEE Trans. Ind. Informat.},
    volume = {18},
    number = {5},
    pages = {3582--3592},
    doi = {10.1109/TII.2021.3116132}
}

@inproceedings{song_non-orthogonal_2021,
    title = {Non-Orthogonal Multiple Access Assisted Federated Learning for {UAV} Swarms: {An} Approach of Latency Minimization},
    booktitle = {Proc. Int. Wireless Commun. Mobile Comput. (IWCMC)},
    author = {Song, Yuxiao and Wang, Tianshun and Wu, Yuan and Qian, Liping and Shi, Zhiguo},
    year = {2021},
    month = jun,
    pages = {1123--1128},
    doi = {10.1109/IWCMC51323.2021.9498792}
}

@inproceedings{mrad_federated_2021,
    title = {Federated Learning for {UAV} Swarms Under Class Imbalance and Power Consumption Constraints},
    booktitle = {Proc. IEEE Global Commun. Conf. (GLOBECOM)},
    author = {Mrad, Ilyes and Samara, Lutfi and Abdellatif, Alaa Awad and {Al-Abbasi}, Abubakr and Hamila, Ridha and Erbad, Aiman},
    year = {2021},
    month = dec,
    pages = {01--06},
    doi = {10.1109/GLOBECOM46510.2021.9685143}
}

@article{he_three-stage_2023,
    title = {Three-Stage {Stackelberg} Game Enabled Clustered Federated Learning in Heterogeneous {UAV} Swarms},
    author = {He, Wenji and Yao, Haipeng and Mai, Tianle and Wang, Fu and Guizani, Mohsen},
    year = {2023},
    month = feb,
    journal = {IEEE Trans. Veh. Technol.},
    doi = {10.1109/TVT.2023.3246636},
    note = {early access}
}

@article{islam_fbi_2022,
    title = {{{FBI}}: {A} Federated Learning-Based Blockchain-Embedded Data Accumulation Scheme Using Drones for {{Internet}} of {{Things}}},
    author = {Islam, Anik and Al Amin, Ahmed and Shin, Soo Young},
    year = {2022},
    month = may,
    journal = {IEEE Wireless Commun. Lett.},
    volume = {11},
    number = {5},
    pages = {972--976},
    doi = {10.1109/LWC.2022.3151873}
}

@article{al-abiad_decentralized_2023-1,
    title = {Decentralized Aggregation for Energy-Efficient Federated Learning via {D2D} Communications},
    author = {{Al-Abiad}, Mohammed S. and Obeed, Mohanad and Hossain, M. J. and Chaaban, Anas},
    year = {2023},
    journal = {IEEE Trans. Commun.},
    note = {early access},
    doi = {10.1109/TCOMM.2023.3253718},
}

@book{hartigan_clustering_1975,
  title={Clustering Algorithms},
  author={Hartigan, John A},
  year={1975},
  publisher={John Wiley \& Sons, Inc.}
}

@inproceedings{mcmahan_communication-efficient_2017,
    title = {Communication-Efficient Learning of Deep Networks from Decentralized Data},
    booktitle = {Proc. Artif. Intell. Stat. (AISTATS)},
    author = {McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and Y Arcas, Blaise Aguera},
    year = {2017},
    month = apr,
    pages = {1273--1282},
    langid = {english}
}

@article{nguyen_federated_2021,
  title = {Federated Learning for {Internet} of {Things}: {A} Comprehensive Survey},
  author = {Nguyen, Dinh C. and Ding, Ming and Pathirana, Pubudu N. and Seneviratne, Aruna and Li, Jun and Vincent Poor, H.},
  year = {2021},
  journal = {IEEE Commun. Surveys Tuts.},
  volume = {23},
  number = {3},
  pages = {1622--1658},
  doi = {10.1109/COMST.2021.3075439}
}

@inproceedings{zhao_dronesense_2022,
  title = {{DroneSense}: {Leveraging} Drones for Sustainable Urban-scale Sensing of Open Parking Spaces},
  booktitle = {Proc. Conf. Comput. Commun. (INFOCOM)},
  author = {Zhao, Dong and Cao, Mingzhe and Ding, Lige and Han, Qiaoyue and Xing, Yunhao and Ma, Huadong},
  year = {2022},
  month = may,
  pages = {1769--1778},
  doi = {10.1109/INFOCOM48880.2022.9796795}
}

@article{xiao_fully_2021,
  title = {Fully Decentralized Federated Learning-Based On-Board Mission for {UAV} Swarm System},
  author = {Xiao, Yue and Ye, Yu and Huang, Shaocheng and Hao, Li and Ma, Zheng and Xiao, Ming and Mumtaz, Shahid and Dobre, Octavia A.},
  year = {2021},
  month = oct,
  journal = {IEEE Commun. Lett.},
  volume = {25},
  number = {10},
  pages = {3296--3300},
  doi = {10.1109/LCOMM.2021.3095362}
}

@article{chen_bdfl_2021,
  title = {{BDFL}: {A} Byzantine-Fault-Tolerance Decentralized Federated Learning Method for Autonomous Vehicle},
  author = {Chen, Jin-Hua and Chen, Min-Rong and Zeng, Guo-Qiang and Weng, Jia-Si},
  year = {2021},
  month = sep,
  journal = {IEEE Trans. Veh. Technol.},
  volume = {70},
  number = {9},
  pages = {8639--8652},
  doi = {10.1109/TVT.2021.3102121}
}

@inproceedings{pokhrel_decentralized_2020,
  title = {A Decentralized Federated Learning Approach for Connected Autonomous Vehicles},
  booktitle = {Proc. IEEE Wireless Commun. Netw. Conf. Workshops (WCNC Wkshps)},
  author = {Pokhrel, Shiva Raj and Choi, Jinho},
  year = {2020},
  month = apr,
  pages = {1--6},
  doi = {10.1109/WCNCW48565.2020.9124733}
}

@article{li_blockchain-based_2021,
  title = {A Blockchain-Based Decentralized Federated Learning Framework with Committee Consensus},
  author = {Li, Yuzheng and Chen, Chuan and Liu, Nan and Huang, Huawei and Zheng, Zibin and Yan, Qiang},
  year = {2021},
  month = jan,
  journal = {IEEE Netw.},
  volume = {35},
  number = {1},
  pages = {234--241},
  doi = {10.1109/MNET.011.2000263}
}

@article{che_decentralized_2022,
  title = {A Decentralized Federated Learning Framework via Committee Mechanism With Convergence Guarantee},
  author = {Che, Chunjiang and Li, Xiaoli and Chen, Chuan and He, Xiaoyu and Zheng, Zibin},
  year = {2022},
  month = dec,
  journal = {IEEE Trans. Parallel Distrib. Syst.},
  volume = {33},
  number = {12},
  pages = {4783--4800},
  doi = {10.1109/TPDS.2022.3202887}
}

@inproceedings{qu_efficient_2021,
  title = {Efficient Edge Intelligence under Clustering for {UAV} Swarm Networks},
  booktitle = {Proc. IEEE Int. Conf. Space-Air-Ground Comput. (SAGC)},
  author = {Qu, Yuben and Dong, Chao and Wu, Tao and Zhuang, Yan and Dai, Haipeng and Wu, Fan},
  year = {2021},
  month = oct,
  pages = {112--117},
  doi = {10.1109/SAGC52752.2021.00026}
}

@article{lecun_gradient-based_1998,
  title = {Gradient-Based Learning Applied to Document Recognition},
  author = {Lecun, Y. and Bottou, L. and Bengio, Y. and Haffner, P.},
  year = {1998},
  month = nov,
  journal = {Proc. IEEE},
  volume = {86},
  number = {11},
  pages = {2278--2324},
  doi = {10.1109/5.726791}
}

@techreport{krizhevsky_learning_2009,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey},
  year={2009},
  institution = {University of Toronto},
}

@article{wang_learning_2021-1,
  title = {Learning in the air: {Secure} Federated Learning for {UAV}-Assisted Crowdsensing},
  author = {Wang, Yuntao and Su, Zhou and Zhang, Ning and Benslimane, Abderrahim},
  year = {2021},
  month = apr,
  journal = {IEEE Trans. Netw. Sci. Eng.},
  volume = {8},
  number = {2},
  pages = {1055--1069},
}

@article{lu_differentially_2020,
  title = {Differentially Private Asynchronous Federated Learning for Mobile Edge Computing in Urban Informatics},
  author = {Lu, Yunlong and Huang, Xiaohong and Dai, Yueyue and Maharjan, Sabita and Zhang, Yan},
  year = {2020},
  month = mar,
  journal = {IEEE Trans. Ind. Informat.},
  volume = {16},
  number = {3},
  pages = {2134--2143},
  doi = {10.1109/TII.2019.2942179}
}

@article{garey_complexity_1976,
  title = {The Complexity of Near-Optimal Graph Coloring},
  author = {Garey, M. R. and Johnson, D. S.},
  year = {1976},
  month = jan,
  journal = {J. ACM},
  volume = {23},
  number = {1},
  pages = {43--49},
  doi = {10.1145/321921.321926},
  urldate = {2023-08-08}
}

@article{pires_broadcast_2019,
  title = {The Broadcast Storm Problem in {FANETs} and the Dynamic Neighborhood-Based Algorithm as a Countermeasure},
  author = {Pires, Rayner M. and Pinto, Alex Sandro Roschildt and Branco, Kalinka Regina Lucas Jaquie Castelo},
  year = {2019},
  journal = {IEEE Access},
  volume = {7},
  pages = {59737--59757},
  doi = {10.1109/ACCESS.2019.2915561}
}

@book{cormen_introduction_2022,
  title = {Introduction to {{Algorithms}}},
  author = {Cormen, Thomas H. and Leiserson, Charles E. and Rivest, Ronald L. and Stein, Clifford},
  year = {2022},
  month = apr,
  publisher = {{MIT Press}},
  googlebooks = {RSMuEAAAQBAJ},
  langid = {english}
}

@article{liu_federated_2021-1,
  title = {Federated Learning in the Sky: {Aerial}-Ground Air Quality Sensing Framework With {UAV} Swarms},
  author = {Liu, Yi and Nie, Jiangtian and Li, Xuandi and Ahmed, Syed Hassan and Lim, Wei Yang Bryan and Miao, Chunyan},
  year = {2021},
  month = jun,
  journal = {IEEE Internet Things J.},
  volume = {8},
  number = {12},
  pages = {9827--9837},
  doi = {10.1109/JIOT.2020.3021006}
}

@article{he_cgan-based_2023,
  title = {{CGAN}-Based Collaborative Intrusion Detection for {UAV} Networks: {A} Blockchain-Empowered Distributed Federated Learning Approach},
  author = {He, Xiaoqiang and Chen, Qianbin and Tang, Lun and Wang, Weili and Liu, Tong},
  year = {2023},
  month = jan,
  journal = {IEEE Internet Things J.},
  volume = {10},
  number = {1},
  pages = {120--132},
  doi = {10.1109/JIOT.2022.3200121}
}

@inproceedings{li_on_2020,
    title={On the Convergence of {FedAvg} on Non-{IID} Data},
    author={Xiang Li and Kaixuan Huang and Wenhao Yang and Shusen Wang and Zhihua Zhang},
    booktitle={Proc. Intl. Conf. Learn. Representations (ICLR)},
    year={2020},
}







